Keystone: An Open Framework for Architecting TEEs

Trusted execution environments (TEEs) are being used in all the devices from embedded sensors to cloud servers and encompass a range of cost, power constraints, and security threat model choices. On the other hand, each of the current vendor-specific TEEs makes a fixed set of trade-offs with little room for customization. We present Keystone -- the first open-source framework for building customized TEEs. Keystone uses simple abstractions provided by the hardware such as memory isolation and a programmable layer underneath untrusted components (e.g., OS). We build reusable TEE core primitives from these abstractions while allowing platform-specific modifications and application features. We showcase how Keystone-based TEEs run on unmodified RISC-V hardware and demonstrate the strengths of our design in terms of security, TCB size, execution of a range of benchmarks, applications, kernels, and deployment models.

==> tables/sel4.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{lcc}
\toprule
\textbf{Group (\sel Test Suite)}  & \textbf{\# Tests} & \textbf{Overhead (\%)}\\
\midrule
SYSCALL             & 15       & 0.01\\
SERSERV\_PARENT     & 10       & 0.67\\
CNODEOP             & 9        & 0.16\\
PAGEFAULT           & 9        & 0.69\\
IPC                 & 9        & 0.74\\
Others 				& 41       & 0.47\\
\bottomrule
\end{tabular}
\caption{
\codename \sel overhead over native execution for the test suite
(total $93$ tests). We group tests by the prefix of each test name. 
}
\label{tab:sel4}
\end{table}

==> v2/chapters/abstract3.tex <==
Trusted execution environments (TEEs) are being used in all the
devices from embedded sensors to cloud servers and encompass a range
of cost, power constraints, and security threat model choices. On the
other hand, each of the current vendor-specific TEEs makes a fixed set
of trade-offs with little room for customization. We present
\codename---the first open-source framework for building customized
TEEs. \codename uses simple abstractions provided by the hardware such
as memory isolation and a programmable layer underneath untrusted
components (e.g., OS). We build reusable TEE core primitives from
these abstractions while allowing platform-specific modifications and
application features. We showcase how \codename-based TEEs run on
unmodified \riscv hardware and demonstrate the strengths of our design
in terms of security, TCB size, execution of a range of benchmarks,
applications, kernels, and deployment models.

==> v2/chapters/ack.tex <==
We thank Srini Devdas and Ilia Lebedev for sharing the Sanctum
codebase and initial discussions. We thank Alexander Thomas and
Stephan Kaminsky for their help in building \codename and Jerry Zhao
for help in running \codename on BOOM. Thanks to the members of UCB
BAR for their help with the \hifivefull and FireSim setup. We thank
Paul Kocher and Howard Wu for their feedback on the early versions of
this draft. Thanks to the Privado team at Microsoft Research for 
sharing the torch code for our case-study. This material is in part
based upon work supported by the National Science Foundation under
Grant No. TWC-1518899 and DARPA N66001-15-C-4066. Any opinions,
findings, and conclusions or recommendations expressed in this
material are those of the author(s) and do not necessarily reflect the
views of the National Science Foundation. Research partially funded by
RISE Lab sponsor Amazon Web Services, ADEPT Lab industrial sponsors
and affiliates Intel, HP, Huawei, NVIDIA, and SK Hynix. Any opinions,
findings, conclusions, or recommendations in this paper are solely
those of the authors and do not necessarily reflect the position or
the policy of the sponsors.

==> v2/chapters/approach.tex <==
\section{\codename Overview}
\label{sec:approach}

We use \riscv to design and build \codename. \riscv is an open ISA
with multiple open-source core implementations~\cite{rocket, boom}. It
currently supports up to three privilege modes: U-mode (user) for
normal user-space processes, S-mode (supervisor) for the kernel, and
M-mode (machine) which can directly access physical resources (e.g.,
interrupts, memory, devices).

\subsection{Design Principles}

We design \programmable TEEs with maximum degrees of freedom and
minimum effort using the following principles.

\paragraph{Leverage programmable layer and isolation primitives below
the untrusted code.}
We design a \securitymonitor (\sm) to enforce TEE guarantees on the
platform using three properties of M-mode: (a) it is programmable by
platform providers and meets our needs for a minimal highest privilege
mode. (b) It controls hardware delegation of the interrupts and
exceptions in the system. All the lower privilege modes can receive
exceptions or use CPU cycles only when the M-mode allows it. (c)
Physical memory protection (PMP), a feature of the \riscv Privileged
ISA~\cite{riscv-priv-110}, enables the M-mode to enforce simple access
policies to physical memory, allowing isolation of memory regions at
runtime or disabling access to memory-mapped control features.

\paragraph{Decouple the resource management and security checks.} The
\sm enforces security policies with minimal code at the highest
privilege. It has few non-security responsibilities. This lowers its
TCB and allows it to present clean abstractions. Our S-mode \runtime
(\rt) and U-mode enclave application (\eapp) are mutually trusting,
reside in enclave address space, and are isolated from the untrusted
OS or other user applications. The \rt manages the lifecycle of the
user code executing in the enclave, manages memory, services syscalls,
etc. For communication with the \sm, the \rt uses a limited set of API
functions via the \riscv supervisor binary interface (SBI) to exit or
pause the enclave (Table~\ref{table:sm-api}) as well as request \sm
operations on behalf of the \eapp (e.g., attestation). Each enclave
instance may choose its own \rt which is never shared with any other
enclave.

\paragraph{Design modular layers.}
\codename uses modularity (\sm, \rt, \eapp) to support a variety of
workloads. It frees \provider{}s and \codenamedev{}s from retrofitting
their requirements and legacy applications into an existing TEE
design. Each layer is independent, provides a security-aware
abstraction to the layers above it, enforces guarantees which can be
easily checked by the lower layers, and is compatible with existing
notions of privilege.

\paragraph{Allow to selectively include TCB only when required.}
\codename can instantiate TEEs with minimal TCB for each of the
specific expected use-cases. The enclave programmer can further
optimize the TCB via \rt choice and \eapp libraries using existing
user/kernel privilege separation. For example, if the \eapp does not
need libc support or dynamic memory management, \codename will not
include them in the enclave. 

\input{chapters/threat_model}

==> v2/chapters/benchmarks.tex <==
\subsection{Benchmarks}
\label{sec:benchmarks}

We use $4$ standard benchmark suites with a mix of CPU, memory, and
file I/O for system-wide analysis: \textbf{Beebs}, \textbf{CoreMark},
\textbf{RV8}, and \textbf{IOZone}. We report the overheads of the
cache partitioning plugin and physical attacker protection with RV8 as
an example of \codename trade-offs. In all the graphs, `other' refers
to the lifecycle costs for enclave creation, destruction, etc. 

\input{figures/breakdown}

\paragraph{Common Operations.}
Figure~\ref{fig:breakdown} shows the breakdown of various enclave
operations. Initial validation and measurement dominate the startup
with $2$M and $7$M cycles/page for FU540 and Rocket-S due to an
unoptimized software implementation of SHA-3~\cite{sha3}. The
remaining enclave creation time totals $20$k-$30$k cycles. Similarly,
the attestation is dominated by the ed25519~\cite{ed25519} signing
software implementation with $0.7$M-$1.6$M cycles. These are both
one-time costs per-enclave and can be substantially optimized in
software or hardware. The most common \sm operation, context switches,
currently take between $1.8$K(FU540)-$2.6$K(Rocket-S) cycles depending
on the platform. Notably, creation and destruction of enclaves take 
longer on the FU540 ($4$-core), which can be attributed to the
multi-core PMP synchronization. 

\input{figures/eval_iozone.tex}

\paragraph{Standard Benchmarks Used as Unmodified \eapp Binaries.}
\textbf{ \em Beebs, CoreMark, and RV8.} As expected, \codename incurs
no meaningful overheads ($\pm 0.7\%$, excluding enclave
creation/destruction) for pure CPU and memory benchmarks.
\\
\textbf{\em IOZone.} All the target files are located on the untrusted
host and we tunnel the I/O system calls to the host application.
Figure~\ref{fig:iozone} shows the throughput plots of common
file-content access patterns. \codename experiences expected high
throughput loss for both write (avg. $36.2\%$) and read (avg.
$40.9.\%$). There are three factors contributing to the overhead: (a)
all the data crossing the privilege boundary is copied an additional
time via the untrusted buffer, (b) each call requires the \rt to go
through the edge call interface, incurring a constant overhead, and
(c) the untrusted buffer contends in the cache with the file buffers,
incurring an additional throughput loss on re-write (avg. $38.0\%$),
re-read (avg. $41.3\%$), and record re-write (avg. $55.1\%$)
operations. Since (b) is a fixed cost per system call, it increases
the overhead for the smaller record sizes.

\paragraph{Cache Partitioning.}
The mix of pure-CPU and large working-set benchmarks in \textbf{RV8}
are ideal to demonstrate cache partitioning impact. For this
experiment, we grant $8$ of the $16$ ways in the FU540 L2 cache to the
enclave during execution (see Figure~\ref{fig:rv8}). Small working-set
tests show low overheads from cache flush on context switches, whereas
large working-set tests (primes, miniz, and aes) show up to $128.19\%$
overhead due to a smaller effective cache. The enclave initialization
latency is unaffected.

\input{figures/eval_cache}

\input{tables/rv8_plugin_overhead}

\paragraph{Physical Attacker Protections.}
We ran the \textbf{RV8} suite with our on-chip execution plugins,
enclave self-paging, page encryption, and a DRAM backing page store 
(Table~\ref{tab:rv8_plugin_overhead}). A few \eapps (\texttt{sha512},
\texttt{dhrystone}), which fit in the $1$MB on-chip memory, incurs no
overhead and are protected even from \attackerphy. For the larger
working-set-size \eapps, the paging overhead increases depending on
the memory access pattern. For example, \texttt{primes} incurs the
largest amount of page faults because it allocates and randomly
accesses a $4MB$ buffer causing a page fault for almost every memory
access. Software-based memory encryption adds $2-4 \times$ more
overhead to page faults. These overheads can be alleviated by the
\codename framework if a larger on-chip memory or dedicated hardware
memory encryption engine is available as we discussed in
Section~\ref{sec:framework}.

==> v2/chapters/casestudies.tex <==
\subsection{Case Studies}
\label{sec:case-studies}

We demonstrate how \codename can be adapted for a varied set of
devices, workloads, and application complexities with three
case-studies: (a) machine learning workloads for the client and
server-side usage, (b) a cryptographic library porting effort for
varied \rts, (c) a small secure computation application written
natively for \codename. The evaluation for these case-studies was 
performed on the \hifive board.

\paragraph{Porting Efforts \& Setup.}
We used the unmodified application code logic, hard-coded all the 
configurations and arguments for simplicity, and statically linked the
binaries against $\tt{glibc}$ or $\tt{musl}$~$\tt{libc}$ supported in
the \eyriert. We ported the widely used cryptographic library
\texttt{libsodium} to both \eyrie and \sel \rt trivially.

\paragraph{Case-study 1: Secure ML Inference with Torch and \eyrie.}
We ran nine Torch-based models of increasing sizes with \eyrie on the
Imagenet dataset~\cite{imagenet} (see Table~\ref{tab:torch}). They
comprise $15.7$ and $15.4$K\loc of TH~\cite{torch-th} and
THNN~\cite{torch-thnn} libraries from Torch compiled with
$\tt{musl}$~$\tt{libc}$. Each model has an additional $230$ to $13.4$
K\loc of model-specific inference code~\cite{privado}. We performed
two sets of experiments: (a) execute the model inference code with
static maximum enclave size; (b) turn on the dynamic resizing plugin
so that the enclave extends its size on-demand when it executes.
Figure~\ref{fig:torch} shows the performance overheads for these two
configurations and non-enclaved execution baseline. 
\input{tables/torch}
\input{figures/torch_graph}
\\
\textbf {\em Initialization Overhead.} is
noticeably high for both static size and dynamic resizing. It is
proportional to the \eapp binary size due to enclave page hashing.
Dynamic resizing reduces the initialization latency by $2.9$\% on
average as the \rt does not map free memory during enclave creation.
\\
\textbf{\em \eapp Execution Overhead.} We report an overhead between
$-3.12\%$(LeNet) to $7.35\%$(Densenet) for all the models with both
static enclave size and dynamic resizing. The cause for this is: (a)
\codename loads the entire binary in physical memory before it beings
\eapp execution, precluding any page faults for zero-fill-on-demand or
similar behavior, so smaller sized networks like LeNet execute faster
in \codename; (b) the overhead is primarily proportional to the number
of layers in the network, as more layers results in more memory
allocations and increase the number of $\tt{mmap}$ and $\tt{brk}$
syscalls. We used a small hand-coded test to verify that \eyrie \rt's
custom $\tt{mmap}$ is slower than the baseline kernel and incurs
overheads. So Densenet, which has the maximum number of layers
($910$), suffers from larger performance degradation. In summary, for
long-running \eapps, \codename incurs a fixed one-time startup cost
and the dynamic resizing plugin is indeed useful for larger \eapps.

\paragraph{Case-study 2: Secure ML with FANN and \sel.}
\codename can be used for small devices such as IoT sensors and
cameras to train models locally as well as flag events with model
inference. We ran FANN, a minimal (8K\loc C/C++) \eapp for embedded
devices with the \sel \rt to train and test a simple XOR network. The
end-to-end execution overhead is $0.36\%$ over running in \sel without
\codename.

\paragraph{Case-study 3: Secure Remote Computation.}
We designed and implemented a secure server \eapp (and remote client)
to count the number of words in a given message. We executed it with
\eyrie and no plugins. It performs attestation, uses libsodium to bind
a secure channel to the attestation report, then polls the host
application for encrypted messages using edge-calls, processes them
inside the enclave, and returns an encrypted reply to be sent to the
client. The \eapp consists of the secure channel code using libsodium
($60$ \loc), the edge-wrapping interface ($45$ \loc), and other logic
($60$ \loc). The host is $270$ \loc and the remote client is $280$
\loc. \codename takes $45$K cycles for a round-trip with an empty
message, secure channel, and message passing overheads. It takes
~$47$K cycles between the host getting a message and the enclave
notifying the host to reply.

==> v2/chapters/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We present \codename, the first framework for \programmable TEEs. With
our modular design, we showcase the use of \codename for several
standard benchmarks and applications on illustrative \rts and various
deployments platforms. \codename can serve as a framework for
research and prototyping better TEE designs.

==> v2/chapters/design2.tex <==
\section{\codename Internals}
\label{sec:internals}

We discuss the \codename design details and the enclave lifecycle. Our
enclave consists of a kernel-like component in the S-mode (the
runtime---\rt), and an application in the U-mode (the enclave
application---\eapp). The \rt and the host OS share a dedicated buffer
that is accessible only to specific \rt functions and the host.

\input{tables/sm_api}

\input{chapters/mem_isolation}

\input{chapters/lifecycle}

\input{figures/mmu_diff}

\input{chapters/mmu}

==> v2/chapters/evaluation2.tex <==
\section{Evaluation}
\label{sec:evaluation}

We aim to answer the following questions in our evaluation:
\begin{enumerate}[label=(\bf{\em RQ\arabic*}), align=left, leftmargin=*] 

\item {\bf Modularity.}
Is the \codename framework viable in different configurations for real
applications?

\item {\bf TCB.}
What is the TCB of \codename-instantiated TEE in various deployment
modes?

\item {\bf Performance.}
How much overhead does \codename add to \eapp execution time?

\item {\bf Real-world Applications.}
Does \codename provide expressiveness with minimal developer efforts
for \eapps?

\end{enumerate} 

\paragraph{Experimental Setup.}
%
We used four different setups for our experiments; the \hifivefull
~\cite{HiFiveUnleashed} with a closed-source \hifivesoc (at 1GHz), and
three open-source \riscv processors: small Rocket (Rocket-S), default
Rocket~\cite{rocket}, and Berkeley Out-of-order Machine
(BOOM)~\cite{boom}. See Table~\ref{tab:hw_configs} for details. We
instantiated the open-source processors on FPGAs using
FireSim~\cite{firesim} which is responsible for emulating the cores at
1GHz. The host OS is buildroot Linux (kernel 4.15). All evaluation was
performed on the \hifive and the data is averaged over $10$ runs
unless otherwise specified.

\input{tables/hw_configs.tex}

\input{chapters/modularity}

\input{chapters/benchmarks}

\input{chapters/casestudies}

==> v2/chapters/framework2.tex <==
\section{\codename Framework}
\label{sec:framework}

Figure~\ref{fig:keystone_workflow} details the steps from \codename
provisioning to \eapp deployment. Independently, the \eapp and the \rt
developers use \codename tools and libraries to write \eapps and
plugins. They can specify the plugins they want to use at the enclave
compile time. \sm plugins that expose additional hardware or security
functionality are determined at compile and provisioning time. We now
demonstrate our various \codename plugins.

\input{figures/keystone_workflow}

\input{chapters/plugins}

\input{chapters/primitives}

==> v2/chapters/implementation2.tex <==
\section{Implementation}
\label{sec:implementation}
%
We implemented our \textbf{\sm} on top of the Berkeley Boot Loader
(bbl)~\cite{bbl-riscv-pk}. It supports M-mode trap handling, boot, and
other features. We simulated the primitives that require hardware
support (randomness, root-of-trust, etc.) and provided well-defined
interfaces. All the plugins in Section~\ref{sec:framework} are
available as compile-time options. Memory encryption is implemented
using software AES-128~\cite{aes-lib} and integrity protection is
partially implemented. We implemented the \textbf{\eyriert} from
scratch in C. We ported the \textbf{\sel microkernel}~\cite{sel4} to
\codename with $290$ \loc modifications to \sel for boot, memory
initialization, and interrupt handling. There are no inherent
restrictions to these two \rts, and we expect future development to
add further options. Our  user-land interface for interactions with
the enclaves is provided via a \textbf{Linux kernel module} that
creates a device endpoint (\texttt{/dev/\codename}).

We provide several libraries (edge-calls, host-side syscall endpoints,
attestation, etc.) in C and C++ for the host, the \eapp, and
interaction with the driver-provided Linux device. Our provided tools
generate the enclave measurements (hashes) without requiring \riscv
hardware, customize the \eyriert, and package the host application,
\eapp{}s, \rt into a single binary. We have a complete top-level build
solution to generate a bootable Linux image (based on the tooling for
the \hifivefull) for QEMU, FPGA softcores, and the \hifive containing
our \sm, the driver, and the enclave binaries. \codename is
open-source and available at \keystonegithub{}.

\paragraph{Writing \eapps.}
The \eapp developers can choose to port their legacy applications 
along with one of the default \rts provided by \codename. This
requires near-zero developer efforts. Alternatively, the developers
can use our SDK to write \eapp specifically for \codename. Lastly, 
\codename supports manually partitioning the applications such that
the security-sensitive parts of the logic execute inside the enclave,
while the rest of the code can execute in the untrusted host. Thus,
\codename framework gives the developers ample flexibility in
designing and implementing \eapps. 

==> v2/chapters/introduction3.tex <==
\section{Introduction}
\label{sec:introduction}

The last decade has seen the proliferation of trusted execution
environments (TEEs) to protect sensitive code and data. All major CPU
vendors have rolled out their TEEs (e.g., ARM TrustZone, Intel
SGX, and AMD SEV) to create a secure execution environment, commonly
referred to as an {\em enclave} ~\cite{sgx, trustzone, amd-sev}. On 
the consumer end, TEEs are now being used for secure cloud
services~\cite{haven, scone}, databases~\cite{enclavedb}, big data
computations~\cite{vc3, m2r, securekeeper}, secure
banking~\cite{droidvault}, blockchain consensus
protocols~\cite{teechain, proof-of-luck, poet}, smart
contracts~\cite{towncrier, ekiden, tesseract}, machine
learning~\cite{sgx-ml, privado}, network middleboxes~\cite{endbox,
vif}, and so on. These use-cases have diverse deployment environments
ranging from cloud servers, client devices, mobile phones, ISPs, IoT
devices, sensors, and hardware tokens.
{\let\thefootnote\relax\footnote{{\codename is available at
\keystoneurl }}}

Unfortunately, each vendor TEE enables only a small portion of the
possible design space across threat models, hardware requirements,
resource management, porting effort, and feature compatibility. When a
cloud provider or software developer chooses a target hardware
platform they are locked into the respective TEE design limitations
regardless of their actual application needs. Constraints breed
creativity, giving rise to significant research effort in working
around these limits. For example, Intel SGXv1~\cite{sgx} requires 
statically sized enclaves, lacks secure I/O and syscall support, and
is vulnerable to significant side-channels~\cite{sgx-explained}. Thus,
to execute arbitrary applications, the systems built on SGXv1 have
inflated the Trusted Computing Base (TCB) and are forced to implement
complex workarounds~\cite{haven, enclavedb, scone, graphene-sgx,
panoply}. As only Intel can make changes to the inherent design
trade-offs in SGX, users have to wait for changes like dynamic
resizing of enclave virtual memory in the proposed
SGXv2~\cite{sgx-dyn-mem}. Unsurprisingly, these and other similar 
restriction have led to a proliferation of TEE re-implementations on
other ISAs (e.g., OpenSPARC~\cite{sp, bastion}, RISC-V~\cite{sanctum,
timberv}). However, each such redesign requires considerable effort
and only serves to create another fixed design point.

In this paper, we advocate that the hardware must provide security
{\em primitives} and not point-wise solutions. We can draw an analogy
with the move from traditional networking solutions to Software
Defined Networking (SDN), where exposing the packet forwarding
primitives to the software has led to far more use-cases and research
innovation. We believe a similar paradigm shift in TEEs will pave the
way for effortless customization. It will allow features and the
security model to be tuned for each hardware platform and use-case
from a common base. This motivates the need for {\em \programmable
TEEs} to provide a better interface between entities that create the
hardware, operate it, and develop applications. \Programmable TEEs
promise quick prototyping, a shorter turn-around time for fixes,
adaptation to threat models, and use-case specific deployment.

The first challenge in realizing this vision is the lack of a
programmable trusted layer below the {\em untrusted} OS. Hypervisor
solutions result in a trusted layer with a mix of security and
virtualization responsibilities, unnecessarily complicating the most
critical component. Firmware and micro-code are not programmable to a
degree that satisfies this requirement. Second, previous attempts at
re-using hardware isolation to provide TEE guarantees do not capture 
the right notion of customization. Specifically, these solutions (e.g.
Komodo~\cite{komodo}, \sel~\cite{sel4}) rely on the underlying
hardware not only for a separation mechanism but also for pre-made
decision about the boundary between what is trusted and untrusted.
They use a verified trusted software layer for customization on top of
this hardware~\cite{komodo}. To overcome these challenges, our insight
is to identify the appropriate hardware memory isolation primitives
and then build a modular software-programmable layer with the
appropriate privileges 

To this end, we propose \codename---the first open-source framework
for building \programmable TEEs. We build \codename on unmodified
\riscv using its standard specifications~\cite{riscv-priv-110} for
physical memory protection (PMP)---a primitive which allows the
programmable machine mode underneath the OS in \riscv to specify
arbitrary protections on physical memory regions. We use this machine
mode to execute a trusted {\em security monitor (SM)} to provide
security boundaries without needing to perform any resource
management. More importantly, enclave operates in its own
isolated physical memory region and has its own {\em
runtime} (\rt) component which executes in supervisor mode and manages
the virtual memory of the enclave. With this novel design, any
enclave-specific functionality can be implemented cleanly by its \rt
while the \sm manages hardware-enforced guarantees. This allows the
enclaves to specify and include only the necessary components. The \rt
implements the functionality, communicates with the \sm, mediates
communication with the host via shared memory, and services {\em
enclave user-code application (\eapp)}.

Our choice of \riscv and the logical separation between \sm and \rt
allows hardware manufacturers, cloud providers, and application
developers to configure various design choices such as TCB, threat
models, workloads, and TEE functionality via compile-time plugins.
Specifically, \codename's \sm uses hardware primitives to provide
in-built support for TEE guarantees such as secure boot, memory
isolation, and attestation. The \rt then provides functionality
plugins for system call interfaces, standard $\tt{libc}$ support,
in-enclave virtual memory management, self-paging, and more inside the
enclave. For strengthening the security, our \sm leverages a highly
configurable cache controller to transparently enable defenses against
physical adversaries and cache side-channels.

We build \codename, the \sm, and an \rt (called \eyrie) which together
allow enclave-bound user applications to selectively use all the above
features. We demonstrate an off-the-shelf microkernel
(\sel~\cite{sel4}) as an alternative \rt. We extensively benchmark
\codename on $4$ suites with varying workloads: RV8, IOZone, CoreMark,
and Beebs. We showcase use-case studies where \codename can be used
for secure machine learning (Torch and FANN frameworks) and
cryptographic tasks (sodium library) on embedded devices and cloud
servers. Lastly, we test \codename on different \riscv systems: the
\hifivefull, $3$ in-order cores and $1$ out-of-order core via FPGA,
and a QEMU emulation---all without modification. \codename is
open-source and available online~\cite{anon-code-release}.

\paragraph{Contributions.} We make the following contributions:
\begin{itemize}

\item{\em Need for \Programmable TEEs.}
We define a new paradigm wherein the hardware
manufacturer, hardware operator, and the enclave programmer can 
tailor the TEE design.

\item{\em \codename Framework.}
We present the first framework to build and instantiate \programmable
TEEs. Our principled way of ensuring modularity in \codename allows us
to customize the design dimensions of TEE instances as per the
requirements.

\item {\em Open-source Implementation.}
We demonstrate the advantages of \codename TEEs which can minimize the
TCB, adapt to threat models, use hardware features, handle workloads,
and provide rich functionality without any micro-architectural changes.
Total TCB of a \codename enclaved application is between $12$-$15$~K
lines of code (\loc), of which the \sm consists of only $1.6$~K\loc
added by \codename.

\item {\em Benchmarking \& Real-world Applications.}
We evaluate \codename on $4$ benchmarks: CoreMark, Beebs, and RV8
($<1\%$ overhead), and IOZone ($40\%$). We demonstrate real-world
machine learning workloads with Torch in \eyrie ($7.35\%$), FANN
($0.36\%$) with \sel, and a \codename-native secure remote computation
application. Finally, we demonstrate enclave defenses for adversaries
with physical access via memory encryption and a cache side-channel
defense.

\end{itemize}

==> v2/chapters/keystone_abstraction.tex <==
\subsection{Entities in TEE Lifecycle}
\label{sec:actors}

We define six logical entities in \programmable TEEs:
\\
\emph{\bf \designer} designs the hardware; designs or modifies
existing SoCs, IP blocks and interactions.
\\
\emph{\bf \manufacturer} fabricates the hardware; assembles them as
per the pre-defined design.
\\
\emph{\bf \provider} purchases manufactured hardware; operates
the hardware; makes it available for use to its customers; configures
the \sm.
\\
\emph{\bf \codenamedev} develops \codename software components
including \sm, \rt, and \eapps; we refer to the programmers who 
develop these specific components as \smdev, \rtdev, \eappdev
respectively. 
\\
\emph{\bf \codenameuser} chooses a \codename configuration of \rt and
an \eapp. They instantiate a TEE which can execute on their choice of
hardware provisioned by the \provider.
\\
\emph{\bf \eappuser} interacts with the \eapp executing in an enclave
on the TEE instantiated using \codename. 
\\
We define these fine-granularity roles for customization options in
\codename. In real-world deployments, a single entity can perform
multiple roles. For example, consider the scenario where Acme Corp.
hosts their website on an Apache webserver executing on Bar Corp.
manufactured hardware in a \codename-based enclave hosted on Cloud
Corp. cloud service. In this scenario, Bar will be the \designer and
\manufacturer; Cloud will be a \provider and can be an \rtdev and
\smdev; Apache developers will be \eappdev; Acme Corp. will be
\codename user, and; the person who uses the website will be the
\eappuser.

==> v2/chapters/lifecycle.tex <==
\subsection{Enclave Lifecycle}
\label{sec:lifecycle}

We summarize the end-to-end life cycle of a \codename enclave. 
Figure~\ref{fig:enclave_lifecycle} shows the key steps in the
enclave lifetime and the corresponding PMP changes.
\input{figures/enclave_lifecycle}
\\
{\bf \em Enclave Creation.}
At creation, \codename measures the enclave memory to ensure that the
OS has loaded the enclave binaries correctly to the physical memory.
\codename uses the initial virtual memory layout for the measurement 
because the physical layout can legitimately vary (within limits)
across different executions. For this, the \sm expects the OS to
initialize the enclave page tables and allocate physical memory for
the enclave. The \sm walks the OS-provided page table and checks if
there are invalid mappings and ensures a unique virtual-to-physical
mapping. Then the \sm hashes the page contents along with the virtual
addresses and the configuration data.
\\
{\bf \em Enclave Execution.} 
The \sm sets the PMP entries and transfers the control to the enclave
entry point.
\\
{\bf \em Enclave Destruction.}
On an OS initiated tear-down, the \sm clears the enclave memory region
before returning the memory to the OS. \sm cleans and frees all the
enclave resources, PMP entries, and enclave metadata.

==> v2/chapters/mem_isolation.tex <==
\subsection{\codename Memory Isolation Primitives}
\label{sec:tee_primitives}

\codename has significantly better modularity and customizability 
because of our conscious design choices. First, we expect the hardware
to provide only simple security primitives and interfaces. Second, we
assign minimum responsibilities of the trusted software components
executing at the highest privilege (e.g., bootloader, \sm). Finally,
we push bulk of the resource management logic either to the untrusted
software or the enclave.

\paragraph{Background: \riscv Physical Memory Protection.}
\codename uses physical memory protection (PMP) feature provided by
\riscv. PMP restricts the physical memory access of S-mode and U-mode
to certain regions defined via {\em PMP entries} (See
Figure~\ref{fig:pmp_full}).\footnote{\texttt{pmpaddr} and
\texttt{pmpcfg} CSRs are used to specify PMP entries} Each PMP entry
controls the U-mode and S-mode permissions to a customizable region of
physical memory.\footnote{Currently processors have up to $16$ M-mode
configurable PMP entries.} The PMP address registers encode the
address of a contiguous physical region, configuration bits specify
the r-w-x permissions for U/S-mode, and two addressing mode bits. PMP
has three addressing modes to support various sizes of regions
(arbitrary regions and power-of-two aligned regions). PMP entries are
statically prioritized with the lower-numbered PMP entries taking
priority over the higher-numbered entries. If any mode attempts to
access a physical address and it does not match any PMP address range,
the hardware does not grant any access permissions.

\paragraph{Enforcing Memory Isolation via \sm.}
PMP makes \codename memory isolation enforcement flexible for three
reasons: (a) multiple discontiguous enclave memory regions can coexist
instead of reserving one large memory region shared by all enclaves;
(b) PMP entries can cover a regions between sizes $4$ bytes or maximum
DRAM size so \codename enclaves utilize page-aligned memory with an
arbitrary size; (c) PMP entries can be dynamically reconfigured during
execution such that \codename can dynamically create a new region or
release a region to the OS.

\input{figures/pmp_full}

During the SM boot, \codename configures the first PMP entry (highest
priority) to cover its own memory region (code, stack, data such as
enclave metadata and keys). The \sm disallows all access to its
memory from U-mode and S-mode using this first entry and configures
the last PMP entry (lowest priority) to cover all memory and with all
permissions enabled. The OS thus has default full permissions to all
memory regions not otherwise covered by a PMP entry.

When a host application requests the OS to create an enclave, the OS
finds an appropriate contiguous physical region. On receiving a valid
enclave creation request, the \sm protects the enclave memory by
adding a PMP entry with all permissions disabled. Since the enclave's
PMP entry has a higher priority than the OS PMP entry (the last in
Figure~\ref{fig:pmp_full}), the OS and other user processes cannot
access the enclave region. A valid request requires that enclave
regions not overlap with each other or with the \sm region.

At a CPU control-transfer to an enclave, the \sm (for the current core
only): (a) enables PMP permission bits of the relevant enclave memory
region; and (b) removes all OS PMP entry permissions to protect all
other memory from the enclave. This allows the enclave to access its
own memory and no other regions. At a CPU context-switch to
non-enclave, the \sm disables all permissions for the enclave region
and re-enables the OS PMP entry to allow default access from the OS.
Enclave PMP entries are freed on enclave destruction.

\paragraph{PMP Enforcement Across Cores.}
Each core has its own complete set of PMP entries. During enclave
creation, \codename adds a PMP entry to disallow everyone from
accessing the enclave. These changes during the creation must be
propagated to all the cores via inter-processor interrupts (IPIs). 
The \sm executing on each of the cores handles these IPIs by removing 
the access of other cores to the enclave. During the enclave
execution, changes to the PMP entries (e.g., context switches between
the enclave and the host) are local to the core executing it and need
not be propagated to the other cores. When \codename destroys or
creates an enclave, all the other cores are notified to update their
PMP entries. There are no other times when the PMPs need to be
synchronized via IPIs.

==> v2/chapters/mmu.tex <==
\subsection{Post-creation In-enclave Page Management}
%
\codename has a different memory management design from the existing
TEEs (see Figure~\ref{fig:mmu_diff}). It uses the OS generated
page-tables for the initialization and then delegates the
virtual-to-physical memory mapping entirely to the enclave during
the execution. Since \riscv provides per-hardware-thread views of the
physical memory via the machine-mode and the PMP registers, it allows
\codename to have multiple concurrent and potentially multi-threaded
enclaves to access the disjoint physical memory partitions. With an
isolated S-mode inside the enclave, \codename can execute its own
virtual memory management which manipulates the enclave-specific
page-tables. Page tables are always inside the isolated enclave memory
space. By leaving the memory management to the enclave we: (a) support
several plugins for memory management which are not possible in any
of the existing TEEs (see Section~\ref{sec:mem_plugins}); (b) remove
controlled side-channel attacks as the host OS cannot modify or
observe the enclave virtual-to-physical mapping.

==> v2/chapters/modularity.tex <==
\subsection{Modularity \& Support}
\label{sec:modularity}

\input{tables/runtime_tcb}

We outline the qualitative measurement of \codename flexibility in 
extending features, reducing TCB, and using the platform features.
Table~\ref{tab:runtime_tcb} shows the TCB breakdown of various
components (required and optional) for the \sm and \eyriert.

\paragraph{Extending \rts.} 
Most of the modifications (e.g., additional edge-call features)
require no changes to the \sm, and the \eappdev may enable them as
needed. Future additions (e.g., ports of interface shields) may be
implemented exclusively in the \rt. We also add support for a new \rt
by porting \sel to \codename and use it to execute various \eapps (See
Section~\ref{sec:case-studies}). \codename passes all the tests in 
\sel suite and incurs less than $1\%$ overhead on average over all
test cases.

\paragraph{Extending the \sm.}
The advantage of an easily modifiable \sm layer is noticeable when the
features require interaction with the core TEE primitives like memory
isolation. The \sm features were able to take advantage of the L2
cache controller on the FU540 to offer additional security protections
(cache-partitioning and on-chip isolation) without changes to the \rt
or \eapp.

\paragraph{TCB Breakdown.}
\codename comprises of the M-mode components (\texttt{bbl} and \sm),
the \rt, the untrusted host application, the \eapp, and the helper
libraries, of which only a fraction is in the TCB. The M-mode
component is $~10.7$ K\loc with a cryptographic library ($4$ K\loc),
pre-existing trap handling, boot, and utilities ($4.7$ K\loc), the \sm
($1.6$ K\loc), and \sm plugins ($400$ \loc).
%
A minimum \eyriert is $1.8$ K\loc, with plugins adding
further code as shown in Table~\ref{tab:runtime_tcb} up to a maximum
\eyriert TCB of $3.6$ K\loc.
%
The current maximum TCB for an \eapp running on our \sm and \eyriert
is thus a total of $~15$ K\loc.
%
TCB calculations were made using \texttt{cloc}~\cite{cloc} and
\texttt{unifdef}~\cite{unifdef}.

==> v2/chapters/plugins.tex <==
\subsection{Enclave Memory Management Plugins}
\label{sec:mem_plugins}

Each enclave can run both S-mode and U-mode code. Thus, it has the
privileges to manage the enclave memory without crossing the
isolation boundaries. By default, \codename enclaves may occupy a
fixed contiguous physical memory allocated by the OS, with a
statically-mapped virtual address space at load time. Although this is
suitable for some embedded applications, it limits the memory usage of
most legacy applications. To this end, we describe several optional
plugins which enable flexible memory management of the enclave.

\paragraph{Free-memory.}
We built a plugin that allows the \eyrie \rt to perform page table
changes. It also lets the enclave reserve physical memory without
mapping it at creation time. This unmapped (hence, free) memory region
is not included in the enclave measurement and is zeroed before
beginning the \eapp execution. The free-memory plugin is required for
other more complex memory plugins.

\paragraph{Dynamic Resizing.}
Statically pre-defined maximum enclave size and subsequent static
physical / virtual memory pre-allocations prevent the enclave from 
scaling dynamically based on workload. It also complicates the process
of porting existing applications to \eapps. To this end, \codename
allows the \eyrie \rt to request dynamic changes to the physical
memory boundaries of the enclave. The \eyrie \rt may request that the
OS make an $\tt{extend}$ SBI call to add contiguous physical pages to
the enclave memory region. If the OS succeeds in such an allocation,
the \sm increases the size of the enclave and notifies the \eyrie \rt
who then uses the free memory plugin to manage the new physical pages.

\paragraph{In-Enclave Self Paging.}
We implemented a generic in-enclave page swapping plugin for the
\eyriert. It handles the enclave page-faults and uses a generic page
backing-store that manages the evicted page storage and retrieval. Our
plugin uses a simple random \eapp-only page eviction policy. It works
in conjunction with the free memory plugin for virtual memory
management in the \eyrie \rt. Put together, they help to alleviate the
tight memory restrictions an enclave may have due to the limited DRAM
or the on-chip memory size~\cite{eleos, varys, cosmix}.

\paragraph{Protecting the Page Content Leaving the Enclave.}
When the enclave handles its own page fault, it may attempt to evict
the pages out of the secure physical memory (either an on-chip memory
or the protected portion of the DRAM). When these pages have to be
copied out, their content needs to be protected. Thus, as part of the
in-enclave page management, we implement a backing-store layer that
can include page encryption and integrity protection to allow for the
secure content to be paged out to the insecure storage (DRAM regions
or disk). The protection can be done either in the software as a part
of the \codename \rt (Figure~\ref{fig:plugin_schematic}(d)) or by a
dedicated trusted hardware unit---a memory encryption engine
(MEE)~\cite{general-purpose-mee}---with an \sm plugin
(Figure~\ref{fig:plugin_schematic}e). Admittedly, this incurs
significant design challenges in efficiently storing the metadata and
performance optimizations. \codename design is agnostic to the
specific integrity schemes and can reuse the existing
mechanisms~\cite{merkletree, bonsaitree}.

\input{figures/plugin_schematic.tex}

\subsection{SM Plugins}
\label{sec:security_plugins}
%
\codename can easily integrate with optional hardware to provide
stronger security guarantees at the cost of various trade-offs. We
demonstrate several SM plugins that can defend the enclave against a
physical attacker or cache side-channel attacks using the \hifivesoc
L2 memory controller. 

\paragraph{Secure On-chip Memory.}
To protect the enclaves against a physical attacker who has access to
the DRAM, we implemented an \emph{on-chip memory} plugin
(Figure~\ref{fig:plugin_schematic}(c)). It allows the enclave to
execute without the code or the data leaving the chip package. On the
\hifivesoc, we dynamically instantiate a scratchpad memory of up to
$2$MB via the L2 memory controller to generate a usable on-chip memory
region. An enclave requesting to run in the on-chip memory loads
nearly identically to the standard procedure with the following
changes: (a) the host loads the enclave to the OS allocated memory
region with modified initial page-tables referencing the final
scratchpad address; and (b) the \sm plugin copies the standard enclave
memory region into the new scratchpad region before the measurement.
Any context switch to the enclave now results in an execution in the
scratchpad memory. This plugin uses only our basic enclave life-cycle
hooks for the platform-specific plugins and does not require further
modification of the \sm. The only other change required was a
modification of the untrusted enclave loading process to make it aware
of the physical address region that the scratchpad occupies. No
modifications to the \eyriert or the \eapps are required.

\paragraph{Cache Partitioning.}
Enclaves are vulnerable to cache side-channel attacks from the
untrusted OS and the applications on the other cores via a shared
cache. To this end, we build a cache partitioning plugin using two
hardware capabilities: (a) the L2 cache controller's
\textit{waymasking} primitive similar to Intel's CAT~\cite{intelCAT};
(b) PMP to way-partition the L2 cache transparently to the OS and the
enclaves. Our plugin enforces effective {\em non-interference} between
the partitioned domains, see Figure~\ref{fig:plugin_schematic}(b).
Upon a context switch to the enclave, the cache lines in the partition
are flushed. During the enclave execution, only the cache lines from
the enclave physical memory are in the partition and are thus
protected by PMP. The adversary cannot insert cache lines in this
partition during the enclave execution due to the line replacement
way-masking mechanism. The net effect is that the adversary
(\attackerscc) gains no information about the evictions, the resident
lines, or the residency size of the enclave's cache. Ways are
partitioned at runtime and are available to the host whenever the
enclave is not executing even if paused.

\subsection{Functionality Plugins}
\label{sec:function_plugins}

\paragraph{Edge Call Interface.}
The \eapp cannot access the non-enclave memory in \codename. If it
needs to read/write the data outside the enclave, the \eyrie \rt
performs {\em edge calls} on its behalf. Our edge call, which is
functionally similar to RPC, consists of an index to a function
implemented in the untrusted host application and the parameters to be
passed to the function. \eyrie tunnels such a call safely to the
untrusted host, copies the return values of the function back to the
enclave, and sends them to the \eapp. The copying mechanism requires
\eyrie to have access to a buffer shared with the host. To enable
this: (a) the OS allocates a shared buffer in the host memory space
and passes the address to the \sm at enclave creation; (b) the \sm
passes the address to the enclave so the \rt may access this memory;
(c) the \sm uses a separate PMP entry to enable OS access to this
shared buffer. All the edge calls have to pass through the \eyriert as
the \eapp does not have access to the shared memory virtual mappings.
This plugin can be used to add support for syscalls, IPC,
enclave-enclave communication, and so on.

\paragraph{Proxied System Calls.}
We allow the proxying of some syscalls from the \eapp to the host
application by re-using the edge call interface. The user host
application then invokes the syscall on an untrusted OS on behalf of
the \eapp, collects the return values, and forwards them to the \eapp.
\codename can utilize existing defenses to prevent Iago
attacks~\cite{iago} via this interface~\cite{besfs, cosmix,
graphene-sgx}.

\paragraph{In-enclave System Calls.}
For appropriate syscalls (e.g., mmap, brk, getrandom), \codename
invokes an \sm interface or executes them in \eyrie to return the
results to the \eapp.

\paragraph{Multi-threading.}
We run multi-threaded \eapps by scheduling all the threads on the same
core. We do not support parallel multi-core enclave execution yet.

==> v2/chapters/primitives.tex <==
\subsection{Other \codename Primitives}
\codename supports following other standard TEE primitives.

\paragraph{Secure Boot.}
A \codename root-of-trust can be either a tamper-proof software (e.g.,
a zeroth-order bootloader) or hardware (e.g., crypto engine). At each
CPU reset, the root-of-trust (a) measures the \sm image, (b) generates
a fresh attestation key from a secure source of randomness, (c) stores
it to the \sm private memory, and (d) signs the measurement and the
public key with a hardware-visible secret. These are standard
operations, can be implemented in numerous
ways~\cite{sanctum-secure-boot,microsemi-secure-boot}. \codename does
not rely on a specific implementation. For completeness, currently,
\codename simulates secure boot via a modified first-stage bootloader
to performs all the above steps.

\paragraph{Secure Source of Randomness.}
\codename provides a secure \sm SBI call, $\tt{random}$, which
returns a $64$-bit random value. \codename uses a hardware source of
randomness if available or can use other well-known
options~\cite{mowery2013welcome} if applicable.

\paragraph{Trusted Timer.}
\codename allows the enclaves to access the read-only
hardware-maintained timer registers via the $\tt{rdcycle}$
instruction. The \sm supports standard timer SBI calls.

\paragraph{Remote Attestation.}
\codename \sm performs the measurement and the attestation based on
the provisioned key. Enclaves may request a signed attestation from
the \sm during runtime. \codename uses a standard scheme to bind the
attestation with a secure channel construction~\cite{komodo,
sanctum-secure-boot} by including limited arbitrary data (e.g.,
Diffie-Hellman key parameters) in the signed attestation report. Key
distribution~\cite{sgx-seal}, revocation~\cite{PKI-CRL}, attestation
services~\cite{intel-attestation-service}, and anonymous
attestation~\cite{direct-anonymous-attestation} are orthogonal
challenges.

\paragraph{Secure Delegation.}
\codename delegates the traps (i.e., interrupts and exceptions) raised
during the enclave execution to the \rt via the interrupt delegation
registers. The \rt invokes the appropriate handlers inside the enclave
for user-defined exceptions and may forward other traps to the
untrusted OS via the \sm.

\paragraph{Monotonic Counters \& Sealed Storage.}
Enclaves may need monotonic counters for protection against rollback
attacks and versioning~\cite{sgx-explained}. \codename can support
monotonic counters by keeping a limited counter state in the \sm
memory. \codename can support sealed storage~\cite{sgx-seal} in the
future.

==> v2/chapters/problem2.tex <==
\section{\Programmable TEEs}
\label{sec:problem}
\input{figures/keystone_overview.tex}

We motivate the need for \programmable TEEs which can adapt to 
various real deployment scenarios, introduce our key actors, and
define our goals.

\subsection{Need for a New Paradigm.}
Current widely-used TEE systems cater to specific and valuable 
use-cases but occupy only a small part of the wide design space (see
Table~\ref{tab:comparison}). Consider the case of heavy server
workload (databases, ML inference, etc.) running in an untrusted cloud
environment. One option is an SGX-based solution which has a large
software stack~\cite{haven, graphene-sgx, scone} to extend the
supported features. On the other hand, a SEV-based solution requires a
complete virtualization stack. If one wants additional defenses
against side-channels, it adds further user-space software mechanisms
for both cases. If we consider edge-sensors or IoT applications, the
available solutions are TrustZone based. While more flexible than SGX
or SEV, TrustZone supports only a single hardware-enforced isolated
domain called the Secure World. Any further isolation needs
multiplexing between applications within one domain with
software-based Secure World OS solutions~\cite{optee}. Thus,
irrespective of the TEE, developers often compromise their design
requirements (e.g., resort to a large TCB solution, limited privilege
domains) or take on the onus of building their custom design.

\paragraph{Hardware-software co-design.}
\codename builds on simple yet elegant primitives. We leverage
multiple well-defined and existing hardware features while allowing
the software layers to manage the complex responsibilities. Previous
works explore the spectrum of tasks the hardware and software should
do. For instance, \sel~\cite{sel4} uses a single isolation domain
exposed by the hardware and performs almost all resource management,
isolation, and security enforcement in a verified software layer.
Komodo uses the two isolation domains provided by ARM TrustZone to
execute multiple isolated domains enforced by formally verified
software. In \codename, we expect arbitrary hardware-isolated domains
whose boundaries can be dynamically configured in the software. With
this novel choice, \codename provides guarantees with minimum trusted
software while allowing the isolated regions to manage themselves.

\input{tables/comparison}

\paragraph{\Programmable TEEs.} 
We define a new paradigm---{\em \programmable TEEs}---to allow
multiple stakeholders to customize a TEE. The hardware manufacturer
only provides basic primitives. Realizing a specific TEE instance
involves the platform provider's choice of the hardware interface, the
trust model, and the enclave programmer's feature requirements. The
entities offload their choices to a framework which plugs in required
components and composes them to instantiate the required TEE. With
this, we bridge the existing gaps in the TEE design space, allow
researchers to independently explore design trade-offs without
significant development effort, and encourage rapid response to
vulnerabilities and new feature requirements.

\paragraph{Trusted Hardware Requirements.}
\codename requires no changes to CPU cores, memory controllers, etc. A
secure hardware platform supporting \codename has several feature
requirements: a device-specific secret key visible only to the trusted
boot process, a hardware source of randomness, and a trusted boot
process. Key provisioning~\cite{sgx-seal} is an orthogonal problem.
For this paper, we assume a simple manufacturer provisioned key.

\input{chapters/keystone_abstraction}

==> v2/chapters/related2.tex <==
\section{Related Work}
\label{sec:related}

\codename is the first framework for customizing TEEs.
Here, we survey existing TEEs and alternative approaches.

\paragraph{TEE Architectures \& Extensions.}
We summarize the design choices of the most recent TEEs and their
extensions in Table~\ref{tab:comparison}.  Of these, three major TEEs
are closely related to \codename: (a) Intel Software Guard Extension
(SGX) executes user-level code in an isolated virtual address space
backed by encrypted RAM pages~\cite{sgx}; (b) ARM TrustZone divides
the memory into two worlds (i.e., normal vs. secure) to run
applications in protected memory~\cite{trustzone}; and (c) Sanctum
uses the memory management unit (MMU) and cache partitioning to
isolate memory and prevent cache side-channel attacks~\cite{sanctum}. 
Several other TEEs explore design layers such as
hypervisors~\cite{hypersentry, hyperwall, trustvisor, cloudvisor,
nohype, overshadow, inktag, terra, sp, xoar, sp3, chaos}, physical
memory~\cite{sanctorum, mi6, bastion, flicker, oasis, trustlite,
aise}, virtual memory~\cite{timberv, iso-x, virtualghost, secureme,
sanctuary}, and process isolation~\cite{aegis, xom, xomos, drawbridge,
secureblue, ostia}. 

\paragraph{Re-purposing Existing TEEs for Modularity.}
One way to meet \codename design goals is to reuse the TEE solutions
available on commodity  CPUs. For each of these TEEs, it is possible
to enable a subset of  programming constructs (e.g., threading,
dynamic loading of binaries) by including a software management
component inside the enclave~\cite{optee, sierratee, t6, graphene-sgx,
haven}. On the other hand, all of the existing TEEs are hardware
extensions which are designed and implemented by the CPU manufacturer.
Thus, they do not allow users to access the programmable interface at
a layer underneath the untrusted OS. One way to simulate the
programmable layer is by adding a trusted hypervisor layer which then
executes an untrusted OS, but this approach inflates the TCB. Lastly,
none of these potential designs allow for adapting to threat models
and workloads.

\paragraph{Differences from Trusted Hypervisor}
\codename executes the enclave logic in the supervisor mode (\rt) and
the user mode (\eapp), while the machine mode code (\sm) merely checks
and enforces isolation boundaries. Although \codename may seem similar
to a trusted hypervisor, it does not implement or perform any resource
management, virtualization, or scheduling in the \sm. It merely checks
if the untrusted OS and the enclave (\rt, \eapp) are managing the
shared resources correctly. Thus, \codename \sm is more analogous to a
reference monitor~\cite{anderson1972computer, GrahamDenning1972}.

\paragraph{TEE Support.}
Several existing works  enhance existing TEE platforms. At the \sm
layer they optimize program-critical tasks~\cite{sanctum, timberv,
tz-rkp}, at \rt they target portability, functionality,
security~\cite{graphene-sgx, panoply, scone, haven, sancus, asylo, t6,
mesatee, optee, hyperapps, flexible-os, ms-openenclave}, and at \eapp
layer they reduce the developer efforts ~\cite{libseal, talos}.
Although these systems are a fixed configuration in the TEE design
space, they  provide valuable lessons for \codename feature design and
future optimization.

\paragraph{Enhancing the Security of TEEs.}
Better and secure TEE design has been a long-standing goal, with 
advocacy for security-by-design~\cite{bootstrap-trust,
seven-properties-highly-secure-devices}. We point out that \codename
is not vulnerable to a large class of side-channel
attacks~\cite{pte-sgx, cca-sgx, pigeonhole} by design, while
speculative execution attacks~\cite{spectre, foreshadow} are limited
to out-of-order \riscv cores (e.g., BOOM) and do not affect most SOC
implementations (e.g., Rocket). \codename can re-use known cache
side-channel defenses~\cite{mi6, dawg} as we demonstrated in
Section~\ref{sec:security_plugins}. Lastly, \codename can benefit from
various \riscv proposals underway to secure IO operations with
PMP~\cite{sifive-tee}. Thus, \codename either eliminates classes of
attacks or allows integration with existing techniques.

\paragraph{Formally Verified Hardware \& Software.}
TEE-like guarantees can be achieved orthogonally by a hardware and
software stack which is formally verified as resistant against all
classes of attacks that TEEs prevent. A careful and ground-up design
with verified components ~\cite{cheriabi,cheri, kami, sel4, certikos,
vale, vale-popl, certicoq, compcert-paper,evercrypt, everest-snapl,
verve, ironclad, deepspec, device-veri, hyperkernel, cogent} may
provide stronger guarantees, and \codename can help to explore
designs which combine these with hardware protection~\cite{komodo,
tap}.

==> v2/chapters/security.tex <==
\section{Security Analysis}
\label{sec:secanalysis}

We argue the security of the enclave, the OS, and the \sm based on the
threat model outlined in Section~\ref{sec:threat_model}.

\subsection{Protection of the Enclave}
\label{sec:enclave_sec}
%
\codename attestation ensures that any modification of the \sm, \rt,
and the \eapp is visible while creating the enclave. During the
enclave execution, any direct attempt by an \attackersw to access the 
enclave memory (cached or uncached) is defeated by PMP. All the
enclave data structures can only be updated in the enclave or the \sm,
both of them are isolated from direct access. Subtle attacks such as
controlled side channels (\attackerccs) are not possible in \codename
because enclaves have dedicated page management and in-enclave page
tables. This ensures that any enclave executing with any \codename
instantiated TEE is always protected against the above attacks.

\paragraph{Mapping Attacks.}
The \rt is trusted, does not intentionally create malicious virtual to
physical address mappings~\cite{inktag} and ensures that the mappings
are valid. The \rt initializes the page tables either during the
enclave creation or loads the pre-allocated (and \sm validated) static
mappings. During the enclave execution, the \rt ensures that the
layout is not corrupted while updating the mappings (e.g., via mmap).
When the enclave gets new empty pages, say via the dynamic memory
plugin, the \rt checks if they are safe to use before mapping them to
the enclave. Similarly, if the enclave is removing any pages, the \rt
scrubs their content before returning them to the OS.

\paragraph{Syscall Tampering Attacks.}
If the \eapp and the \rt invoke untrusted functions implemented in the
host process and/or execute the OS syscalls, they are susceptible to
Iago attacks and system call tampering attacks~\cite{iago,
ports-garfinkel}. \codename can re-use the existing shielding systems
~\cite{scone, besfs, graphene-sgx} as plugins to defend the enclave 
against these attacks.

\paragraph{Side-channel Attacks.}
\codename thwarts cache side-channel attacks
(Section~\ref{sec:security_plugins}). Enclaves do not share any state
with the host OS or the user application and hence are not exposed to
controlled channel attacks. The \sm performs a clean context switch
and flushes the enclave state (e.g., TLB). The enclave can defend
itself against explicit or implicit information leakage via the SM or
the edge call API with known defenses~\cite{msr-pldi16, moat}. Only
the \sm can see other enclave events (e.g., interrupts, faults), these
are not visible to the host OS. Timing attacks against the \eapp are
out of scope.

\subsection{Protecting the Host OS}
\label{sec:os_sec}
%
\codename \rts execute at the same privilege level as the host OS,
so an \attackersw is our case is stronger than in SGX. We ensure that
the host OS is not susceptible to new attacks from the enclave because
the enclave cannot: (a) reference any memory outside its allocated
region due to the \sm PMP-enforced isolation; (b) modify page tables
belonging to the host user-level application or the host OS; (c) 
pollute the host state because the \sm performs a complete context
switch (TLB, registers, L1-cache, etc.) when switching between an
enclave and the OS; (d) DoS a core as the \sm watchdog timer assures
that the enclave returns control to the OS.

\subsection{Protection of the \sm}
\label{sec:sm_sec}
The \sm naturally distrusts all the lower-privilege software
components (\eapp{}s, \rt{}s, host OS, etc.). It is protected from an
\attackersw because all the \sm memory is isolated using PMP and is
inaccessible to any enclave or the host OS. The \sm SBI is another
potential avenue of attack. \codename's \sm presents a narrow,
well-defined SBI to the S-mode code. It does not do complex resource
management and is small enough to be formally verified~\cite{komodo,
serval}. The \sm is only a reference monitor, it does not require
scheduled execution time, so an \attackerdos is not a concern. The \sm
can defend against an \attackerscc and an \attackersct with known
techniques~\cite{time-sc-survey, dawg}.

\subsection{Protection Against Physical Attackers}
\label{sec:phy_attacker}

\codename can protect against a physical adversary by a combination of
plugins and a proposed modification to the bootloader. Similar to
\cite{chen2008scratchpad}, we use a scratchpad to store the decrypted
code and data, while the supervisor mode component (\eyrie plugins)
handles the page-in and page-out.

\textbf{The enclave} itself is protected by the on-chip memory plugin
(in \sm) and the paging plugins (in \eyrie), with encryption and
integrity protection on the pages leaving the on-chip memory. The page
backing-store is a standard PMP protected physical memory region now
containing only the encrypted pages, similar in concept to the SGX
EPC. This fully guarantees the confidentiality and integrity of the
enclave code and data from an attacker with complete DRAM control. 

\textbf{The \sm} should be executed entirely from the on-chip memory.
The \sm is statically sized and has a relatively small in-memory
footprint ($<150$Kb). On the \hifivesoc, this would involve
repurposing a portion of the L2 loosely-integrated memory (LIM) via a
modified trusted bootloader.

With all of these plugins and techniques in place, the only content
present outside of the chip package is either untrusted (host, OS,
etc.) or is encrypted and integrity protected (e.g., swapped enclave
pages). \codename accomplishes this with no hardware modifications.

==> v2/chapters/threat_model.tex <==
\subsection{Threat Model}
\label{sec:threat_model}

The \codename framework trusts the PMP specification as well as the
PMP and \riscv hardware implementation to be bug-free. The
\codenameuser trusts the \sm only after verifying if the \sm
measurement is correct, signed by trusted hardware, and has the
expected version. The \sm only trusts the hardware, the \rt trusts the
\sm, the \eapp trusts the \sm and the \rt.

\paragraph{Adaptive Threat Model.} 
\codename can operate under diverse threat models, each requiring
different defense mechanisms. For this reason, we outline all the
relevant attackers for \codename. We allow the selection of a sub-set
of these attackers based on the scenario. For example, if the user is
deploying TEEs in their own private data centers or home appliances, a
physical attacker may not be a realistic threat and \codename can be
configured to operate without physical adversary protections.

\paragraph{Attacker Models.}
\codename protects the confidentiality and integrity of all the
enclave code and data at all points during execution. We define four
classes of attackers who aim to compromise our security guarantees:
\\
A {\bf \em physical attacker} \attackerphy can intercept, modify, or
replay signals that leave the chip package. We assume that the
physical attacker does not affect the components inside the chip
package. \attackerphc is for confidentiality, \attackerphi is for
integrity.
\\
A {\bf \em software attacker} \attackersw can control host applications,
the untrusted OS, network communications, launch adversarial enclaves,
arbitrarily modify any memory not protected by the TEE, and
add/drop/replay enclave messages. 
\\
A {\bf \em side-channel attacker} \attackersc can glean information by
passively observing interactions between the trusted and the
untrusted components via the cache side-channel (\attackerscc), the
timing side-channel (\attackersct) or the control channel
(\attackerccs).
\\
A {\bf \em denial-of-service attacker} \attackerdos can take down the
enclave or the host OS. \codename allows these attacks against
enclaves as the OS can refuse services to user applications at any
time.
 
\paragraph{Scope.}
\codename currently has no meaningful mechanisms to protect against
speculative execution attacks~\cite{spectre, foreshadow, zombieload,
ridl, fallout, boom-speculative}. We recommend \codename users to
avoid deployments on out-of-order cores. Existing and future defenses
against this class of attacks can be retrofitted into
\codename~\cite{mi6, invisispec}. \codename does not natively protect
the enclave or the \sm against timing side-channel attacks. \sm, \rt,
and \eapp programmers should use existing software solutions to mask
timing channels~\cite{time-sc-survey} and \manufacturer{}s can supply
timing side-channel resistant hardware~\cite{dawg}. The \sm exposes a
limited API to the host OS and the enclave. We do not provide
non-interference guarantees for this API~\cite{komodo, nickel}.
Similarly, the \rt can optionally perform untrusted system calls into
the host OS. We assume that the \rt and the \eapp have sufficient
checks in place to detect Iago attacks via this untrusted
interface~\cite{besfs, cosmix, graphene-sgx}, and the \sm, \rt, and
\eapp are bug-free.

==> v2/figures/breakdown.tex <==
\begin{figure}
\centering
\includegraphics[width=0.398\columnwidth]{figures/breakdown/hash}
\label{fig:breakdown_hash}
\includegraphics[width=0.592\columnwidth]{figures/breakdown/breakdown}
\caption{
Breakdown of the operations during the enclave life-cycle. (a) shows
the enclave validation and the hashing duration, and (b) shows the
breakdown of other operations. (b) does not include the duration of
size-dependent operations such as the measurement in \texttt{create}
(Shown in (a)) and the memory cleaning in \texttt{destroy} (4K-11K
cycles/page).
}
\label{fig:breakdown}
\end{figure}

==> v2/figures/enclave_lifecycle.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{figures/enclave_lifecycle_fig.pdf}
\caption{
Lifecycle of an enclave. The enclave memory and the corresponding PMP
entry status (accessible or not) are shown per each operation. For
PMP status, \textit{This} means the PMP status of the core performing
the operation and \textit{Others} is PMP of other cores.
}
\label{fig:enclave_lifecycle}
\end{figure}

==> v2/figures/eval_cache.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{figures/benchmarks/benchmark-cache.pdf}
\caption{
Total execution time comparison for the RV8 benchmarks. Each bar
consists of the duration of the application (\texttt{user} or
\texttt{eapp}), and the other overheads (\texttt{other}). \codename
(\texttt{\codename}) and \codename with cache partitioning plugin
(\texttt{\codename-cache}) are compared with the native execution in
Linux (\texttt{base}).
}
\label{fig:rv8}
\end{figure}

==> v2/figures/eval_iozone.tex <==
\begin{figure}
\includegraphics[width=0.95\columnwidth]{figures/iozone/writer_report.pdf}
\includegraphics[width=0.95\columnwidth]{figures/iozone/reader_report.pdf}
\caption{
IOZone file operation throughput in \codename for various file and
record sizes (e.g., r8 represents 8KB record). We only show write and
read results due to limited space.
}
\label{fig:iozone}
\end{figure}

==> v2/figures/keystone_overview.tex <==
\begin{figure}
\includegraphics[width=0.99\columnwidth]{figures/overview_fig.pdf}
\caption{
\codename overview of the system setup and privilege levels. Includes
components such as untrusted host processes, the untrusted OS, the
security monitor, and multiple enclaves (each with a runtime and an
\eapp).}
\label{fig:keystone_overview}
\end{figure}

==> v2/figures/keystone_workflow.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{figures/workflow_fig.pdf}
\caption{ End-to-end Overview of \codename Framework. 
\ding{182} The platform provider configures the \sm. 
\ding{183} \codename compiles and generates the \sm boot image. 
\ding{184} The platform provider deploys the \sm. 
\ding{185} The developer writes an \eapp and configures the enclave. 
\ding{186} \codename builds the binaries and computes their 
measurements. 
\ding{187} The untrusted host binary is deployed to the machine. 
\ding{188} The host deploys the \rt and the \eapp and initiates the 
enclave creation.
\ding{189} A remote verifier can perform the attestation based on a 
known platform specifications, the keys, and the \sm/enclave measurements.}
\vspace{-12pt}
\label{fig:keystone_workflow}
\end{figure}

==> v2/figures/mmu_diff.tex <==
\begin{figure}
\center
\includegraphics[width=0.97\columnwidth]{figures/mmu_diff_fig.pdf}
\caption{
Memory Management Designs (the shaded area is untrusted).
(a) Intel SGX: the untrusted OS manages the memory and translates
virtual-to-physical address. (b) Komodo: the page-tables are inside
the enclave but the monitor creates the mappings. (c) \codename:
delegates page management to enclave with its own page table. (d) XEN:
the hypervisor performs the page management, there are two page tables
in this setup.
}
\label{fig:mmu_diff}
\end{figure}

==> v2/figures/plugin_schematic.tex <==
\begin{figure}
\center
\includegraphics[width=\columnwidth]{figures/plugin_schematic_fig.pdf}
\caption{\codename memory Model for the combination of various plugins.
 \textbf{$\varnothing$}: no plugin,
 \textbf{C}: cache partitioning, \textbf{O}: on-chip scratchpad,
 \textbf{P}: enclave self-paging, \textbf{E}: software memory 
 encryption
 \textbf{E$_{HW}$}: hardware memory encryption.
}
\label{fig:plugin_schematic}
\end{figure}


==> v2/figures/pmp_full.tex <==
\begin{figure}
\includegraphics[width=0.99\columnwidth]{figures/pmp_full_fig.pdf}
\caption{
\keystone's use of \riscv PMP for the flexible, dynamic memory
isolation. The SM uses a few PMP entries to guard its own memory
(\texttt{SM}), enclave memory regions ($\tt{E1}$, $\tt{E2}$),  and the
untrusted buffer ($\tt{U1}$). On enclave entry, the SM will
reconfigure the PMP such that the enclave can only access its own
memory ($\tt{E1}$) and the enclave's untrusted buffer ($\tt{U1}$).
}
\vspace{-10pt}
\label{fig:pmp_full}
\end{figure}


==> v2/figures/torch_graph.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{figures/benchmarks/benchmark-dyn.pdf}
\caption{ Comparison of inferencing duration for various Torch models
with and without dynamic resizing. Each bar consists of the duration
of the application (\texttt{user} or \texttt{eapp}), and the other
overheads (\texttt{other}). \codename (\texttt{\codename}) and
\codename with the dynamic resizing plugin (\texttt{\codename-dyn})
are compared with the native execution in Linux (\texttt{base}).
}
\label{fig:torch}
\end{figure}

==> v2/tables/comparison.tex <==
\begin{table*}[]
\centering
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{clcccccccccc}
\hline
\textbf{} & \multicolumn{1}{c}{\textbf{System}} & 
\begin{tabular}{@{}c@{}}\textbf{Software}\\ \textbf{Adversary} \\ \textbf{Protection}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Physical} \\ \textbf{Adversary} \\ \textbf{Protection}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Side Ch}\\ \textbf{Adversary} \\ \textbf{Protection}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Control Ch} \\ \textbf{Adversary} \\ \textbf{Protection}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Low} \\ \textbf{SW} \\ \textbf{TCB}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{No} \\ \textbf{HW} \\ \textbf{Mods}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Flexible} \\ \textbf{Resource} \\ \textbf{Mgmt}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Range} \\ \textbf{of Apps} \\ \textbf{Supported}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Supports} \\ \textbf{High} \\ \textbf{Expr}\end{tabular} & 
\begin{tabular}{@{}c@{}}\textbf{Low} \\ \textbf{Porting} \\ \textbf{Effort}\end{tabular} \\ \hline \addlinespace[0.2cm]
 & SGX~\cite{sgx} & \compfull & \compfull & \compnone & \compnone & \compfull $^{\textasteriskcentered}$  & \compnone & \compnone & \compnone & \compnone & \compnone \\
 & Haven~\cite{haven} & \compfull & \compfull & \compnone & \compnone & \compnone & \compfull & \comppart & \comppart & \compfull & \compfull \\
 & Graphene-SGX~\cite{graphene-sgx} & \compfull & \compfull & \compnone & \compnone & \compnone & \compfull & \comppart & \comppart & \compfull & \compfull \\
 & Scone~\cite{scone} & \compfull & \compfull & \compnone & \compnone & \comppart & \compfull & \compnone & \comppart & \compfull & \comppart \\
\multirow{-5}{*}{\ver{Intel}} & Varys~\cite{varys} & \compfull & \compfull & \compfull & \comppart & \comppart & \compnone & \compnone & \comppart & \compfull & \comppart \\ \hline \addlinespace[0.15cm]
 & TrustZone~\cite{trustzone} & \compfull & \compnone & \compnone & \compnone & \comppart & \compnone & \compfull & \compfull & \compfull & \compnone \\
 & Komodo~\cite{komodo} & \compfull & \compfull & \compnone & \compfull & \comppart & \compfull & \comppart & \compfull & \comppart & \compfull \\
 & OP-TEE~\cite{optee} & \compfull & \compfull & \compnone & \compnone & \compnone & \compfull & \compfull & \compfull & \compfull & \compfull \\
\multirow{-4}{*}{\ver{ARM}} & Sanctuary~\cite{sanctuary} & \compfull & \compnone & \comppart & \compnone & \compnone & \compfull & \comppart & \compfull & \compfull & \compfull \\ \hline \addlinespace[0.15cm]
 & SEV~\cite{amd-sev} & \comppart & \comppart & \compnone & \compnone & \compfull & \compnone & \compfull & \compfull & \compfull & \compfull \\
\multirow{-2}{*}{\ver{AMD}} & SEV-ES~\cite{amd-sev-es} & \compfull & \compfull & \compnone & \compnone & \compfull & \compnone & \compfull & \compfull & \compfull & \compfull \\ \hline \addlinespace[0.15cm]
 & Sanctum~\cite{sanctum} & \compfull & \compnone & \compfull & \compfull & \comppart & \compnone & \comppart & \comppart & \comppart & \compfull \\
 & TIMBER-V~\cite{timberv} & \compfull & \compfull & \compnone & \compnone & \compfull & \compnone & \compfull & \comppart & \compfull & \comppart \\
 & MultiZone~\cite{multizone} & \compfull & \compfull & \compfull & \compfull & \comppart & \compfull & \compnone & \compnone & \compnone & \comppart \\
\multirow{-4}{*}{\ver{RISC-V}} & \cellcolor[HTML]{EFEFEF}\textbf{\codename (This paper)} & \cellcolor[HTML]{EFEFEF}\compfull & \cellcolor[HTML]{EFEFEF}\compfull & \cellcolor[HTML]{EFEFEF}\compfull & \cellcolor[HTML]{EFEFEF}\compfull & \cellcolor[HTML]{EFEFEF}\comppart & \cellcolor[HTML]{EFEFEF}\compfull & \cellcolor[HTML]{EFEFEF}\compfull & \cellcolor[HTML]{EFEFEF}\compfull & \cellcolor[HTML]{EFEFEF}\comppart & \cellcolor[HTML]{EFEFEF}\compfull \\ \hline
\end{tabular}%
}
\vspace{10pt}
\caption{Trade-offs in existing TEEs and extensions.
%
\textbf{C1-2}: Category and specific systems.
%
\compfull, \comppart, \compnone ~represent best to least adherence to
the property in the column respectively.
%
\textbf{C3-6}: resilience against software adversary, hardware
adversary, side-channel adversary, control-channel adversary
respectively; the symbols indicates complete protection,
only confidentiality protection, and no protection respectively. 
%
\textbf{C7}: zero, thousands of \loc, millions of \loc of TCB. 
\textasteriskcentered ~represents that although the software TCB is
zero/low, the size of the trusted firmware and microcode is still
significantly large.
%
\textbf{C8}: zero or non-zero hardware / micro-architectural modifications.
% 
\textbf{C9}: 
allows the enclave to do self resource management with complete, partial, or no flexibility.
%
\textbf{C10}: the range of applications supported are maximum;
specific class; only written from scratch. 
%
\textbf{C11}: expressiveness includes forking, multi-threading,
syscalls, shared memory; partial; none of these.
%
\textbf{C12}: developer effort for porting is zero (unmodified
binaries); partial (compiling and / or configuration files);
substantial (significant re-writing).} 
\label{tab:comparison}
\end{table*}

==> v2/tables/hw_configs.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{3}{*}{\textbf{Platform}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Core}}} & \multicolumn{2}{c}{\textbf{Cache Size}} & \multicolumn{2}{c}{\textbf{Latency}} & \multicolumn{2}{c}{\textbf{\# of TLB}} \\ 
 & \multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{(KB)}} & \multicolumn{2}{c}{\textbf{(cycles)}} & \multicolumn{2}{c}{\textbf{Entries}} \\ \cmidrule(l){2-9} 
 & \textbf{\#} & \textbf{Type} & \textbf{L1-I/D} & \textbf{L2} & \textbf{L1} & \textbf{L2} & \textbf{L1} & \textbf{L2} \\ \midrule
\textbf{Rocket-S} & 1 & in-order & 8/8 & 512 & 2 & 24 & 8 & 128 \\ 
\textbf{Rocket} & 1 & in-order & 16/16 & 512 & 2 & 24 & 32 & 1024 \\ 
\textbf{BOOM} & 1 & OoO & 32/32 & 2048 & 4 & 24 & 32 & 1024 \\
\textbf{FU540} & 4 & in-order & 32/32 & 2048 & 2 & 12-15* & 32 & 128 \\ \bottomrule
\end{tabular}
\vspace{5pt}
\caption{
Hardware specification for each platform. L2 cache latency in FU540
(*) is based on estimation.
}
\vspace{-10pt}
\label{tab:hw_configs}
\end{table}

==> v2/tables/runtime_tcb.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}


% Got numbers with
%%% No features (base minus edge?) (inc syscall nums (550), reduce to 250 in report since 2x count
% unifdef -UIO_SYSCALL_WRAPPING -ULINUX_SYSCALL_WRAPPING -UUSE_FREEMEM -UENV_SETUP -UDYN_ALLOCATION -UINTERNAL_STRACE -UDEBUG -UPAGING -m *.c *.h *.S
% cloc --exclude-lang="Bourne Shell","Bourne Again Shell","m4","Markdown","make"  .
% 2296
%%% Freemem (sub from base) (INCLUDES paging 270)
% unifdef -UIO_SYSCALL_WRAPPING -ULINUX_SYSCALL_WRAPPING -DUSE_FREEMEM -UENV_SETUP -UDYN_ALLOCATION -UINTERNAL_STRACE -m *.c *.h *.S
% cloc .
% 2871
%%% dyn alloc, use clock git diffing
% cloc --diff  --git master dev-dyn-alloc
% 100?
%%% Edgecall lib (inc syscall nums)
% cloc .
% 845
%%% Syscall support (sub from base)
% 2490
%%% IO Syscall support (sub from base)
% 2573
%%% libc env setup (sub from base)
% 2328
%%% Final counts in table CUT the syscall_nums (from edge and base, 550lines)

%%% SM numbers
%%% dyn
%
%%% Edgecall
% estimated from looking at utm handling code
%%% cache part
% cloc platform/fu540/
%%%

\begin{table}[]
\footnotesize
\centering
\begin{tabular}{lrr}
\toprule
\multicolumn{1}{c}{\textbf{Component}} & \multicolumn{1}{c}{\textbf{Runtime}} & \multicolumn{1}{c}{\textbf{\sm}} \\ \midrule
Base 			& 1800  & 1100 \\
Memory Isolation	& ---   &  500 \\
Free Memory         	&  300  & ---  \\
Dynamic Memory      	&  100  &   70 \\
Edge-call Handling  	&  300  &   30 \\
Syscalls            	&  450  & ---  \\
$\tt{libc}$ Environment &   50  & ---  \\
IO Syscall Proxying 	&  300  & ---  \\
Cache Partitioning  	& ---   &  300 \\
In-enclave Paging  	& 300   &  --- \\
On-chip Memory   	& ---   &  50  \\
\bottomrule
\end{tabular}
\vspace{10pt}
\caption{TCB Breakdowns (in \loc) for \eyrie \rt and \sm features.}
\vspace{-20pt}
\label{tab:runtime_tcb}
\end{table}


==> v2/tables/rv8_plugin_overhead.tex <==
\begin{table}[]
\footnotesize
\centering
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{lrrrrl}
\toprule
\textbf{} & \multicolumn{4}{c}{\textbf{Overhead (\%)}} &\multirow{1}{*}{\textbf{\# of Page}} 
\\ \cline{1-5}  
\textbf{Plugins} & \textbf{$\varnothing$}     & \textbf{C}    & \textbf{O, P}   & \textbf{O, P, E} & \textbf{Faults}\\
\textbf{Adversary} & 
$\mathsf{A}_{SW,Cntrl}$\xspace & 
$\mathsf{A}_{SW,SC}$\xspace & 
$\mathsf{A}_{SW,SC}$\xspace &
$\mathsf{A}_{SW,SC,Phy_C}$\xspace & \textbf{(O, P)}  \\
\hline %\midrule
primes&   -0.9&   40.5&   65475.5&  * &   $66\times 10^6$ \\
miniz&   0.1&   128.5&   80.2&   615.5&   18341 \\
aes&   -1.1&   66.3&   1471.0&   4552.7&   59716 \\
bigint&   -0.1&   1.6&   0.4&   12.0&   168 \\
qsort&   -2.8&   -1.3&   12446.3&   26832.3&   285147 \\
sha512&   -0.1&   0.3&   -0.1&   -0.2&   0 \\
norx&   0.1&   0.9&   2590.1&   7966.4&   58834 \\
dhrystone&   -0.2&   0.3&   -0.2&   0.2&   0 \\
\bottomrule
\end{tabular}
}
\vspace{10pt}
\caption{Overhead of various plugins on RV8 benchmarks over native execution. 
\textbf{$\varnothing$}: no plugin, 
\textbf{C}: cache partitioning, 
\textbf{O}: on-chip scratch pad execution ($1$MB),
\textbf{P}: enclave self-paging,
\textbf{E}: software-based memory encryption.
*: does not complete in \textasciitilde$10$ hrs.
}
\label{tab:rv8_plugin_overhead}
\end{table}

==> v2/tables/sel4.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{lcc}
\toprule
\textbf{Group (\sel Test Suite)}  & \textbf{\# Tests} & \textbf{Overhead (\%)}\\
\midrule
SYSCALL             & 15       & 0.01\\
SERSERV\_PARENT     & 10       & 0.67\\
CNODEOP             & 9        & 0.16\\
PAGEFAULT           & 9        & 0.69\\
IPC                 & 9        & 0.74\\
Others 				& 41       & 0.47\\
\bottomrule
\end{tabular}
\caption{
\codename \sel overhead over native execution for the test suite
(total $93$ tests). We group tests by the prefix of each test name. 
}
\label{tab:sel4}
\end{table}

==> v2/tables/sm_api.tex <==
\begin{table}[]
\centering
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Caller}     & \textbf{SM API} & \textbf{Description}              \\ \midrule
\multirow{5}{*}{OS} & create          & Validate, and measure the enclave \\
                    & run             & Start enclave and boot RT         \\
                    & resume          & Resume enclave execution          \\
                    & destroy         & Release enclave memory            \\
                    \midrule
\multirow{4}{*}{RT} & stop            & Pause enclave execution           \\
                    & exit            & Terminate the enclave             \\
                    & attest          & Get a signed attestation report   \\
                    & random          & Get secure random values          \\ \midrule 
OS \& RT 			& plugin*         & Call SM plugins (e.g., dynamic resizing) \\
                    \bottomrule
\end{tabular}%
}
\vspace{10pt}
\caption{The SBI API functions (SBI) provided by the \codename SM. 
* indicates that the SBI is provided by an optional SM plugin.}
\vspace{-10pt}
\label{table:sm-api}
\end{table}

==> v2/tables/torch.tex <==
\begin{table}[]
\footnotesize
\centering
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\# of \\ Layers\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}\# of\\ Param\end{tabular}}}  & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}App\\ LOC\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Binary\\Size\end{tabular}}}  & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Memory\\Usage\end{tabular}}}  \\ \midrule
Wideresnet   & 93   & 36.5M   & 1625  & 140MB  & 384MB  \\
Resnext29    & 102  & 34.5M   & 1910  & 123MB  & 394MB  \\
Inceptionv3  & 313  & 27.2M   & 5359  &  92MB  & 475MB  \\
Resnet50     & 176  & 25.6M   & 3094  &  98MB  & 424MB  \\
Densenet     & 910  &  8.1M   & 13399 &  32MB  & 570MB  \\
VGG19        & 55   & 20.0M   & 1088  &  77MB  & 165MB  \\
Resnet110    & 552  &  1.7M   & 9528  &   7MB  &  87MB  \\
Squeezenet   & 65   &  1.2M   & 914   &   5MB  &  52MB  \\
LeNet        & 12   &   62K   &	230   &  0.4MB &   2MB  \\
\bottomrule
\end{tabular}
\vspace{10pt}
\caption{Summary of the Torch Models. The model specification, 
workload characteristics, binary object size, and the total
enclave memory usage.}
\label{tab:torch}
\end{table}
